The Shirley reduced basis: a reduced order model for plane-wave DFT

The Shirley reduced basis (SRB) represents the periodic parts of Bloch functions as linear combi- nations of eigenvectors taken from a coarse sample of the Brillouin zone, orthogonalized and reduced through proper orthogonal decomposition. We describe a novel transformation of the self-consistent density functional theory eigenproblem from a plane-wave basis with ultra-soft pseudopotentials to the SRB that is independent of the k-point. In particular, the number of operations over the space of plane-waves is independent of the number of k-points. The parameter space of the transformation is explored and suitable defaults are proposed. The SRB is shown to converge to the plane-wave solution. For reduced dimensional systems, reductions in computational cost, compared to the plane-wave calculations, exceed 5x. Performance on bulk systems improves by 1.67x in molecular dynamics-like contexts. This robust technique is well-suited to efficient study of systems with strin- gent requirements on numerical accuracy related to subtle details in the electronic band structure, such as topological insulators, Dirac semi-metals, metal surfaces and nanostructures, and charge transfer at interfaces with any of these systems. The techniques used to achieve a k-independent transformation could be applied to other computationally expensive matrix elements, such as those found in density functional perturbation theory and many-body perturbation theory.

==> figs/kg_line.tex <==
\begin{tikzpicture}[]

\draw [<->] (-.5,0) -- coordinate(x axis mid) (16.5,0);
\draw (1,4pt) -- (1,-4pt) node[anchor=north] {0};
\draw (5,4pt) -- (5,-4pt) node[anchor=north] {1};
\draw (9,4pt) -- (9,-4pt) node[anchor=north] {2};
\draw (13,4pt) -- (13,-4pt) node[anchor=north] {3};
\pause

\draw [dashed] ( 1,2pt) -- ++ (0,16pt) node[anchor=south] {$k_0$};
\draw [dashed] ( 2,2pt) -- ++ (0,32pt) node[anchor=south] {$k_1$};
\draw [dashed] ( 3,2pt) -- ++ (0,48pt) node[anchor=south] {$k_2$};
\draw [dashed] ( 4,2pt) -- ++ (0,64pt) node[anchor=south] {$k_3$};

\pause

\draw [dashed] ( 5,2pt) -- ++ (0,16pt) node[anchor=south] {$k_0+g_1$};
\draw [dashed] ( 9,2pt) -- ++ (0,16pt) node[anchor=south] {$k_0+g_2$};
\draw [dashed] (13,2pt) -- ++ (0,16pt) node[anchor=south] {$k_0+g_3$};
\pause

\draw [dashed] ( 6,2pt) -- ++ (0,32pt) node[anchor=south] {$k_1+g_1$};
\draw [dashed] (10,2pt) -- ++ (0,32pt) node[anchor=south] {$k_1+g_2$};
\draw [dashed] (14,2pt) -- ++ (0,32pt) node[anchor=south] {$k_1+g_3$};
\pause

\draw [dashed] ( 7,2pt) -- ++ (0,48pt) node[anchor=south] {$k_2+g_1$};
\draw [dashed] (11,2pt) -- ++ (0,48pt) node[anchor=south] {$k_2+g_2$};
\draw [dashed] (15,2pt) -- ++ (0,48pt) node[anchor=south] {$k_2+g_3$};
\pause

\draw [dashed] ( 0,2pt) -- ++ (0,64pt) node[anchor=south] {$k_3+g_{-1}$};
\draw [dashed] ( 8,2pt) -- ++ (0,64pt) node[anchor=south] {$k_3+g_1$};
\draw [dashed] (12,2pt) -- ++ (0,64pt) node[anchor=south] {$k_3+g_2$};
\draw [dashed] (16,2pt) -- ++ (0,64pt) node[anchor=south] {$k_3+g_3$};

\end{tikzpicture}


